Graph Sampling with Distributed In-Memory Dataflow Systems

Given a large graph, a graph sample determines a subgraph with similar characteristics for certain metrics of the original graph. The samples are much smaller thereby accelerating and simplifying the analysis and visualization of large graphs. We focus on the implementation of distributed graph sampling for Big Data frameworks and in-memory dataflow systems such as Apache Spark or Apache Flink. We evaluate the scalability of the new implementations and analyze to what degree the sampling approaches preserve certain graph metrics compared to the original graph. The latter analysis also uses comparative graph visualizations. The presented methods will be open source and be integrated into Gradoop, a system for distributed graph analytics.

==> algorithms/alg_vertex_compute.tex <==
\begin{algorithm}[h]
  \caption{Random Walk - Gelly Compute}\label{alg:vertexcompute}
  \begin{algorithmic}[1]
  	\Require{$\mathcal{G}$, $s \in [0,1]$, $j \in [0,1]$}
    \State $\mathcal{V}_M \gets \emptyset$ \Comment{set of sampled vertices}
    \State $v_W \in V_\mathcal{G}$  \Comment{randomly selected start vertex}
    \Repeat{}
      \State $\mathcal{P}^k \gets \mathcal{G}.\textbf{flatmap}(\textit{report})$
      \State $\phi^k_w \gets \mathcal{P}^k.\textbf{combine}(\textit{count})$
    \Until{$|\mathcal{V}_M| < |V_G| \times s$}  \\
    \Return{$\mathcal{G}_M$}
  \end{algorithmic}
\end{algorithm}
